Pick the Largest Margin for Robust Detection of Splicing

Despite advancements in splicing detection, practitioners still struggle to fully leverage forensic tools from the literature due to a critical issue: deep learning-based detectors are extremely sensitive to their trained instances. Simple post-processing applied to evaluation images can easily decrease their performances, leading to a lack of confidence in splicing detectors for operational contexts. In this study, we show that a deep splicing detector behaves differently against unknown post-processes for different learned weights, even if it achieves similar performances on a test set from the same distribution as its training one. We connect this observation to the fact that different learnings create different latent spaces separating training samples differently. Our experiments reveal a strong correlation between the distributions of latent margins and the ability of the detector to generalize to post-processed images. We thus provide to the practitioner a way to build deep detectors that are more robust than others against post-processing operations, suggesting to train their architecture under different conditions and picking the one maximizing the latent space margin.

==> 4_comparison.tex <==



\subsection{Comparison with classical atomistic strategies}

We propose here to compare the operational regrets obtained for each target of our universe given different strategies : 

\begin{itemize}


    \item Using a relevant source for each target image with the help of a multi-classifier trained to recognize the most representatives sources of our universe.
    \item Applying a majority vote to choose one relevant source for the target among the most representatives ones.
    \item Selecting the source that minimizes the $\ell^2_{CG}$ distance w.r.t. the operational set.
    \item Selecting the source that minimizes the $\mathrm{MMD}$ w.r.t. the operational set.
    \item Selecting the source that minimizes the $\mathrm{NSCD}$ w.r.t. the operational set.

\end{itemize}


Instead of using $10^3$ sources for the majority vote and the multi-classifier, which would severely degrade the performances due to a high number of candidates, we use our methodology from~\cite{wifs2022} to extract a small subset of representatives sources that can achieve less than 5\% regret for all targets. In practice, this enables to work on only 8 %powerful 
sources in terms of generalization. Focusing on only these sources, the efficiency of these strategies is preserved while minimizing space and computation demands. 
Moreover, because there exist sources that are very close to each other, we want to evaluate our metric-based methods only on pairs of source/target which are enough different from each other. %and because this closeness introduces bias into the metrics relying on distances between source and target samples (e.g. the $\ell^2_{CG}$ and the $\mathrm{MMD}$). 
To address the bias induced by evalution on too close pairs
%this potential bias, we are removing 
we remove candidates %from consideration 
if their $\mathrm{MMD}$ is below the 1st decile $Q(10\%)$ of the $\mathrm{MMD}$ distribution that is invariant to operational balancing. This is done for the 3 last strategies to make a fair comparison. The two first strategies use representatives to select sources and are immune to this bias. %This ensures that we are not mistakenly considering sources extremely close to the target, which is not a realistic scenario. 
Moreover, in our evaluations the sources will always have an equal proportion of cover and stego meanwhile the operational set will present different balancing.

We present, in Table~\ref{tab:comparison}, the statistical information relative to the distribution of regrets obtained following the different strategies.
Concerning the two first strategies, the majority vote is less satisfying compared to the others meanwhile the multi-classifier is among the best in terms of efficiency and invariance to the operational balancing. However, this particular strategy cruelly lacks of interpretability. 

On the other side, due to the invariance to cover stego balancing from the $\mathrm{MMD}$ and the $\mathrm{NSCD}$, it is not surprising to see very similar regret distributions in the 3 cases. The strategy using the $\ell^2$-norm is simple and already reasonable in many of the cases. However, its effectiveness depends on the cover stego balance. In the case where the operational target is made up of an equal proportion of covers and stegos, there is about 20\% of regrets observed higher than 5\% using this strategy whereas this lowers to 9\% with the $\mathrm{MMD}$ and 2\% with the $\mathrm{NSCD}$. It is worth mentioning that theoretically, there are situations where the $\mathrm{NSCD}$ is very low and the regret is high. One such example is when the target stems from a significant shift in the source manifold. Curiously, such cases are not present in our experiments. %After the bias removal, sources with very low $\mathrm{NSCD}$ with the target may not exist depending on the target, which explains the biggest regrets observed here with the $\mathrm{NSCD}$. 


\subsection{Geometry-based optimization}

Since the $\mathrm{NSCD}$ exhibits a high correlation with the regret, we suggest leveraging it as a valuable tool for data-adaptation. The methodology involves starting with a set of RAW images, performing image development operations, computing the $\mathrm{NSCD}$ in relation to the target, and repeating the development to minimize the $\mathrm{NSCD}$ as much as possible. To optimize the selection of development parameters, we propose employing well-established heuristics such as simulated annealing. By testing this straightforward concept in our universe, specifically focusing on the most challenging scenarios where regrets are higher than 20\%, we observe satisfying results presented in Table~\ref{tab:geomoptim}. Out of the 30,000 cases studied, 88\% of the regrets obtained at the end of the optimization are below 5\%, with a maximum iteration count of 100. These experiments clearly indicate the superiority of this strategy over the previous method, which required the creation of $10^3$ sources. 

\begin{table}[h!]
    \begin{tabular}{|c|c|c|}
    \hline
    \textbf{Number of scenarios} & \textbf{\%($R_{final}\leq 5$)} & \textbf{Maximum iteration count} \\ \hline
    30.000                                                & 88\%                                      & 100                                    \\ \hline
    \end{tabular}
    \caption{Regret distribution outcomes of geometry-based optimization.}
    \label{tab:geomoptim}
\end{table}

\vspace*{-0.6cm}

\subsection{Impact of the target size}
%Even if our results are very encouraging, 
With a very limited amount of target samples, the $\mathrm{NSCD}$ is not well estimated and leads to wrong source selections as shown in Table \ref{tab:nbsamples}. For instance, we observe that $\mathrm{NSCD}$ is not anymore invariant to operational balancing and much less useful when the amount of target samples is equal to 10. Speaking more generally, we observed through several experiments that when the noise level in the target rises, approximating the manifold becomes more challenging and a larger number of samples is required to achieve accurate estimation of the $\mathrm{NSCD}$. Here, we observe still an acceptable performance with 100 samples (with only $4.6\%$ regrets higher than 5\%). 

    \begin{table}[h!]
        \begin{tabular}{|c|cc|cc|cc|}
        \hline
                               & \multicolumn{2}{c|}{\textbf{Only Covers}}                                           & \multicolumn{2}{c|}{\textbf{Only Stegos}}                                           & \multicolumn{2}{c|}{\textbf{Mix}}                                                   \\ \hline
        \textbf{$N_{samples}$} & \multicolumn{1}{c|}{\textit{\textbf{Max}}} & \textit{\textbf{\%(R\textgreater{}5)}} & \multicolumn{1}{c|}{\textit{\textbf{Max}}} & \textit{\textbf{\%(R\textgreater{}5)}} & \multicolumn{1}{c|}{\textit{\textbf{Max}}} & \textit{\textbf{\%(R\textgreater{}5)}} \\ \hline
        10                     & \multicolumn{1}{c|}{27}                    & 45\%                                   & \multicolumn{1}{c|}{27}                    & 44\%                                   & \multicolumn{1}{c|}{24}                    & 23.8\%                                 \\ \hline
        100                    & \multicolumn{1}{c|}{16}                    & 2.7\%                                  & \multicolumn{1}{c|}{16}                    & 2.5\%                                  & \multicolumn{1}{c|}{16}                    & 4.6\%                                  \\ \hline
        500                    & \multicolumn{1}{c|}{16}                    & 1.6\%                                  & \multicolumn{1}{c|}{16}                    & 1.5\%                                  & \multicolumn{1}{c|}{16}                    & 2\%                                    \\ \hline
        \end{tabular}
        \caption{Information about the regret distributions obtained selecting the source minimizing the $\mathrm{NSCD}$ according to the number of operational samples available. The column max is for the maximum regret observed according to each case.}
        \label{tab:nbsamples}
        \end{table}



% Additionally, the computation time for computing the NSCD increases due to the O($N^3$) complexity of the PCA algorithm used in the process. Lastly, it is important to acknowledge the difficulty in accurately optimizing the search for a suitable source using the NSCD, particularly when starting from a source that is ill-suited for the target and lacking information about the practical processing operations carried out by the steganographer. That being said, the NSCD continues to demonstrate its efficiency in determining the lack of usefulness of a source for the generalization to a target. 
% \NPB{I'm not sure that this section is useful, I would insiste on the impact of the number of observations, with a small tabular on the other side.}



